Smaller Is Better: An Analysis of Instance Quantity/Quality Trade-off in Rehearsal-based Continual Learning

The design of machines and algorithms capable of learning in a dynamically changing environment has become an increasingly topical problem with the increase of the size and heterogeneity of data available to learning systems. As a consequence, the key issue of Continual Learning has become that of addressing the stability-plasticity dilemma of connectionist systems, as they need to adapt their model without forgetting previously acquired knowledge. Within this context, rehearsal-based methods i.e., solutions in where the learner exploits memory to revisit past data, has proven to be very effective, leading to performance at the state-of-the-art. In our study, we propose an analysis of the memory quantity/quality trade-off adopting various data reduction approaches to increase the number of instances storable in memory. In particular, we investigate complex instance compression techniques such as deep encoders, but also trivial approaches such as image resizing and linear dimensionality reduction. Our findings suggest that the optimal trade-off is severely skewed toward instance quantity, where rehearsal approaches with several heavily compressed instances easily outperform state-of-the-art approaches with the same amount of memory at their disposal. Further, in high memory configurations, deep approaches extracting spatial structure combined with extreme resizing (of the order of $8\times8$ images) yield the best results, while in memory-constrained configurations where deep approaches cannot be used due to their memory requirement in training, Extreme Learning Machines (ELM) offer a clear advantage.

==> misc/abstract_pelosin.tex <==
\hide{
As data flow and heterogeneity increases in our world, we are compelled to build smarter machines able to learn in a dynamically changing environment. The requirements of such systems should resemble human intelligence, that is, the tendency to incrementally adapt and not forget the knowledge acquired in the past. Continual Learning constitutes a step towards such direction by addressing the stability-plasticity dilemma of connectionist systems. In our study we propose an analysis of memory compression techniques useful in rehearsal based methods i.e. in solutions where the learner exploits its memory to revisit past data. In particular we investigate complex instance compression techniques such as deep encoders but also trivial approaches such as image resizing and dimensionality reductions. Our findings suggest that compression schemes easily allow a simple baseline to achieve and outperform state of the art performances in all the major datasets used in literature. We also found that in low budget memory and constrained machine resources scenarios, Extreme Learning Machines (ELM) constitute an optimal approach where all other competitors fail.}

==> misc/stuff.tex <==
 In (a) first we consider the image $x_{i}$ as a flattened vector $v_{i}$, then we compute the compression by projecting $v_{i}$ through a quasi-orthogonal random matrix $Q$. The incremental learner is an MLP, thus creating an Extreme Learning Machine \cite{huang_universal_2006}. In (b) we apply, to each image, an encoder/compressor $\psi(\cdot)$ to the images, giving us a vectorial latent representation of the data. In the experiments we studied VAE \cite{DBLP:journals/corr/KingmaW13} and a MBT \cite{DBLP:conf/nips/MinnenBT18} as $\psi(\cdot)$ which are pretrained on a never seen dataset. In (d) we define $\phi(\cdot)$ to be a pretrained ResNet18 \cite{DBLP:conf/cvpr/HeZRS16} cut up to a predefined layer, the output is a small resized noise-free image. In (c) we study the simplest compression technique i.e. the resize of data, where each image is downscaled with bilinear interpolation. In each different image we show that if the compression is in a vector form we use a MLP as learning model otherwise we use a ResNet18.
 
 
 @article{knnsv, 
    author = {Jia, Ruoxi and Dao, David and Wang, Boxin and Hubis, Frances Ann and Gurel, Nezihe Merve and Li, Bo and Zhang, Ce and Spanos, Costas and Song, Dawn}, 
    title = {Efficient Task-Specific Data Valuation for Nearest Neighbor Algorithms}, 
    year = {2019}, 
    journal = {Proc. VLDB Endow.}, 
}


@InProceedings{taskfree_aljundi,
author = {Aljundi, Rahaf and Kelchtermans, Klaas and Tuytelaars, Tinne},
title = {Task-Free Continual Learning},
booktitle = {CVPR},
year = {2019}
}


@inproceedings{encoder,
  title={Encoder based lifelong learning},
  author={Rannen, Amal and Aljundi, Rahaf and Blaschko, Matthew B and Tuytelaars, Tinne},
  booktitle={CVPR},
  year={2017}
}
